Sapphire: Querying RDF Data Made Simple

RDF data in the linked open data (LOD) cloud is very valuable for many different applications. In order to unlock the full value of this data, users should be able to issue complex queries on the RDF datasets in the LOD cloud. SPARQL can express such complex queries, but constructing SPARQL queries can be a challenge to users since it requires knowing the structure and vocabulary of the datasets being queried. In this paper, we introduce Sapphire, a tool that helps users write syntactically and semantically correct SPARQL queries without prior knowledge of the queried datasets. Sapphire interactively helps the user while typing the query by providing auto-complete suggestions based on the queried data. After a query is issued, Sapphire provides suggestions on ways to change the query to better match the needs of the user. We evaluated Sapphire based on performance experiments and a user study and showed it to be superior to competing approaches.

==> sections/02_Preliminaries.tex <==
\section{Preliminaries: RDF and SPARQL}
\label{sec:preliminaries}

%The Resource Description Framework (RDF)~\cite{RDF} is a framework for
%representing information on the web.
RDF~\cite{RDF} data follows a simple graph-based data model.
An RDF graph consists of a set of subject-predicate-object \textit{triples}.
Each
%RDF
triple represents a directed edge from a vertex representing the
subject to a vertex representing the object.
The label on the edge is the predicate, which represents the relationship
between the subject and the object.
Resources (instances, classes, or relations) in the RDF graph are
identified by Uniform Resource Identifiers (URIs).
Literals in RDF are strings of characters, and only objects can be
literals.
Formally, assume two countably infinite disjoint sets, $U$ for URIs and
$L$ for literals. Any RDF triple $(s,p,o) \in U \times U \times (U \cup
L)$.
The following is an example of a set of triples about the movie ``The
Godfather'' from DBpedia in Turtle format~\cite{Turtle}:

\begin{verbatim}
Prefix dbp: <http://dbpedia.org/property/> .
Prefix dbo: <http://dbpedia.org/ontology/> .
Prefix res: <http://dbpedia.org/resource/> .
res:The_Godfather
  dbp:name "The Godfather"@en ;
  dbo:director res:Francis_Ford_Coppola ;
  dbo:distributor res:Paramount_Pictures .
\end{verbatim}

This example shows three triples. The subject is the URI representing the
movie.
The predicates are URIs representing relations to other entities or
literals
(name, director, and distributor).
One object is a literal 
(for the name relation), and the
other two are URIs of other entities.

%\subsection{SPARQL}
%\label{subsec:sparql}
%With the adoption of the RDF as an abstraction to publish data comes the
%challenge of providing an interface for accessing this data.
SPARQL is the standard query language for RDF~\cite{SPARQL}.
The basic building blocks of a SPARQL query are \emph{graph patterns}, and \emph{conditions} applied over
these patterns.
%~\cite{Arenas2016}.
Formally, assume another countably infinite set $V$ for variables, which start with a question mark. This set is disjoint from $U$ and $L$. 

A condition is inductively defined as follows:
\squishlist
\item if $?x, ?y \in V$ and $a \in (U \cup L)$, then $?x$ $op$ $a$ and $?x$ $op$ $?y$, where $op$ is a binary operator, are conditions,
\item if $R_{1}$ and $R_{2}$ are conditions, then $(\neg R_{1})$, $(R_{1} \vee R_{2})$, and $(R_{1} \wedge R_{2})$ are conditions.
\squishend

A graph pattern is inductively defined as follows:
\squishlist
\item a triple from $(U \cup V) \times (U \cup V) \times (U \cup V \cup L)$ is a graph pattern,
\item if $P_{1}$ and $P_{2}$ are graph patterns, then ($P_{1} \wedge
  P_{2}$), ($P_{1}$ OPT  $P_{2}$), ($P_{1}$ UNION  $P_{2}$), and ($P_{1}$
  MINUS  $P_{2}$) are graph patterns (see~\cite{SPARQL} for a definition of
  these operators),
\item if $P$ is a graph pattern and $R$ is a condition, then ($P$ FILTER $R$) is a graph pattern.
\squishend

The goal is to match the graph patterns in the SPARQL query to the queried
datasets to find values that can be associated with the variables in the
graph pattern. These values are the answers to the SPARQL query. 
If a pattern has a FILTER, then only the matches that satisfy the condition
are retained.
SPARQL also has other features such as solution modifiers, e.g., DISTINCT,
and aggregation.
% that are used to control the answers returned as answers to the graph
% pattern matching and applying aggregate functions,
% respectively~\cite{SPARQL}.

% Following is an example of a SPARQL query that finds the name of the director of the movie ``The Godfather'' and other movies by the same director, given that they were distributed by the same studio:
% \begin{verbatim}
% PREFIX dbp: <http://dbpedia.org/property/>
% PREFIX foaf: <http://xmlns.com/foaf/0.1/>
% PREFIX dbo: <http://dbpedia.org/ontology/>
% SELECT DISTINCT ?directorName ?movies WHERE {
%   ?movie dbp:name "The Godfather"@en.
%   ?movie dbp:director ?director.
%   ?movie dbo:distributor ?godFatherDistr.
%   ?director foaf:name ?directorName.
%   ?movies dbp:director ?director.
%   ?movies dbo:distributor ?otherDistr.
%   FILTER (?godFatherDistr = ?otherDistr).
% }
% \end{verbatim}


==> sections/Dijkstras.tex <==
\section{Bi-directional Dijkstra Algorithm}
\label{app:biDijkstras}

In this appendix, we present more details about the bi-directional Dijkstra shortest path algorithm that is used by the QSM.
In a graph $G = (V, E)$ (directed or undirected), the Dijkstra shortest path algorithm finds the shortest path between a source vertex $s$ and a destination vertex $d$ by starting from $s$, and at each step greedily expanding the vertex with the minimum tentative distance $dist(v)$. The bi-directional Dijkstra shortest path algorithm works in the same fashion, except that it alternates its steps between $s$ and $d$. That is, in one step, the vertex with the minimum \emph{forward} weight $d_{f}$ is expanded, and in the next step the vertex with the minimum \emph{reverse} weight $d_{r}$ is expanded.

The stopping condition of this algorithm is not as simple as the forward Dijkstra algorithm.
An intuitive stopping condition is to stop when a vertex $v$ is about to be expanded for the second time (expanded by forward search and then by backward search, or vice versa).
However, in some cases this condition can return a path that is not the shortest between $s$ and $d$. The reason for this is that $v$ may not actually be on the shortest path. A correct stopping condition is to stop when it is guaranteed that no shorter path will be found. This can be done by maintaining the total cost (weight) of the shortest path found so far $\mu$, which is updated whenever an edge $(v,z)$ is visited as part of expanding $v$ in forward search, and $z$ is already expanded in reverse search. In such a case, $\mu$ is updated if $d_{f}(v) + w_{vz} + d_{r}(z) < \mu$, where $w_{vz}$ is the weight of the edge connecting $v$ and $z$. A similar condition is applied in reverse search (when $v$ is already expanded). The algorithm stops if $top_{f} + top_{r} \geq \mu$, where $top_{f}$ and $top_{r}$ are the top heap values for vertices to be expanded in the forward and reverse directions, respectively. For more details, please refer to~\cite{Goldberg2005}.

While the time complexity of the bi-directional Dijkstra algorithm is the same as the forward Dijkstra algorithm, in practice, the bi-directional Dijkstra algorithm is more efficient, and its efficiency increases as the branching factor of the vertices in the graph increases. If $B$ is the branching factor of the vertices in $G$, in the worst case, the Dijkstra algorithm will visit $B^{k}$ vertices, where $k$ is the number of vertex expansions needed to reach $d$. However, in the bi-directional Dijkstra algorithm, the number of visited vertices is $2B^{\frac{k}{2}}$. This is important for us since visiting vertices requires issuing SPARQL queries.


==> sections/FinerResults.tex <==
\section{Fine-Grained Results}
\label{app:finerResults}

\begin{figure*}[t]
\centering
\includegraphics[height=4.5cm,width=1.8\columnwidth]{figures/finePercentage.eps}
\caption{The percentage of each query from being answered.}
\label{fig:finePercentage}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[height=4.5cm,width=1.8\columnwidth]{figures/fineAttempts.eps}
\caption{The average number of attempts for each query.}
\label{fig:fineAttempts}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[height=4.5cm,width=1.8\columnwidth]{figures/fineTime.eps}
\caption{The average time spent on each query.}
\label{fig:fineTime}
\end{figure*}


In Section~\ref{sec:evaluation}, we discussed how Sapphire performs in terms of finding answers to the questions in Appendix~\ref{app:querySet}. We reported the average numbers obtained per category for better readability. In this section, we report the average numbers for each question in Appendix~\ref{app:querySet}. Figure~\ref{fig:finePercentage} shows the average percentage of time a query has been answered in the evaluation. Figure~\ref{fig:fineAttempts} shows the average number of attempts made for each question. Figure~\ref{fig:fineTime} shows the average time spent on each query.

==> sections/SapphirePerformance.tex <==
\section{Performance of \system Components}
\label{app:performance}

\subsection{QCM Performance}

\begin{figure}[t]
\centering
\includegraphics[height=3.5cm,width=0.9\columnwidth]{figures/HitRatio.pdf}
\caption{Hit ratio of the suffix tree.}
\label{fig:hitRatio}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[height=3.5cm,width=0.9\columnwidth]{figures/scalability.pdf}
\caption{Searching for literals in the bins.}
\label{fig:scalability}
\end{figure}

In this appendix, we present an additional set of experiments that studies the performance of \system. It is important for the QCM to provide auto-complete suggestions with very low response time in order to guarantee an interactive experience for users.
We measure the response time of the QCM based on the logs of user interaction from our user study.
Two components contribute to the response time of the QCM: the lookup in the suffix tree, and the sequential search in the bins of literals.
We have found that the total response time of these two components is, on average, 0.16 seconds when including 10000 significant literals in the suffix tree and using 8 cores for the sequential search in the literal bins. This response time is low enough to provide a  good interactive experience for the users of \system~\cite{Miller1968}.

We now study the two components of this response time in more detail. 
We have found that a lookup operation in the suffix tree takes approximately 0.25 milliseconds, regardless of the number of literals that are indexed.
This response time is certainly low enough for an interactive user experience.
Recall that matches in the suffix tree are returned immediately to the user before the search in the bins of literals begins.
Thus, having a hit (match) in the suffix tree greatly enhances the interactive experience, since the user sees auto-complete suggestions very quickly.
Even if these suggestions are not chosen by the user, they still give an impression of a responsive system.
Therefore, a higher hit ratio in the suffix tree is better for interactive response of the QCM.
The hit ratio (fraction of query terms for which a match is found in the suffix tree) depends on the number of literals included in the suffix tree.
Figure~\ref{fig:hitRatio} shows this hit ratio as the number of literals in the suffix tree increases.
The hit ratio flattens starting around 5000 literals, so 10000
literals is sufficient for the best achievable performance.
%: almost half the terms see instant suggestions based on a hit in the suffix tree.

 
The second component of the QCM response time is the sequential search in the literal bins.
Recall that the bins to be searched are filtered based on the length of the term entered by the user.
We have found that, on average, this filtering eliminates 46\% of the literals to be searched.
When including 10000 significant literals in the suffix tree, the search in the remaining literals of DBpedia takes 0.6 seconds when using 1 core, and 0.16 seconds when using 8 cores.
The drop in response time of this search as the number of cores increases is shown in Figure~\ref{fig:scalability} , along with the ideal drop in response time.
The figure shows that the parallelization approach adopted by the QCM is effective, since the actual drop in response time is close to the ideal drop.

%This experiment shows that \system can achieve near-instant interactive response time with limited computing and storage resources (8 cores). Even with minimal resources (1 core), the response time is a reasonable 0.6 seconds.
%To guarantee the best performance,
The takeaway of this experiment is that as many literals as possible should
be included in the suffix tree for best performance.  For literals not in the suffix tree, \system can effectively utilize  more cores to reduce response time. 

%In this section, we evaluate the performance of the Query Completion Module (QCM). It is important to provide the user with an almost instant-response interface to use in \system. It is suggested that for systems that interact with a human to have a ceiling of a response time of 2 seconds, and that 0.1 seconds can be considered ``instant''~\cite{Miller1968}. In \system, we have an average total response time (returning suggestions from index and bins) of 0.16 seconds when indexing the 10000 most significant literals and using 8 cores in the QCM. We refer to the total response time as just response time. Following, we evaluate how changes in these parameters affect the instant-response of \system.

%On one core while indexing the most significant 10000 literals, the QCM response time is 0.6 seconds as shown in Figure~\ref{fig:scalability}. This response time makes \system usable, but cannot be considered instant. Figure~\ref{fig:scalability} shows that when more cores are utilized in the lookup process to find suggestions to complete the query terms, the response time is reduced proportionally. It drops to 0.16 seconds when 8 cores are used, which is very close to being instant.

%In our experiments, we find that a lookup task in the suffix tree takes approximately 0.25 milliseconds, regardless of how many literals are indexed. This means that if there are $n$ hits (matches) in the suffix tree, they are returned instantly. If $n > k$, this means that no secondary index lookup is needed in the secondary index. If $n < k$, the rest of $k-n$ remaining suggestions are found by performing a secondary index lookup. This means that the hit ratio can be considered as the probability of returning a match instantly. While reiterating over the fact that the suffix tree match does not necessarily be what the user is looking for, it is always useful to instantly return a candidate match. Figure~\ref{fig:hitRatio} shows the hit ratio of the suffix tree. That is, how often a match for the typed query term is found in the suffix tree. The figure shows that for as low as 1000 literals indexed, a hit ratio of almost 30\% is achieved, 45\% is achieved when indexing 5000 literals, and almost 50\% when indexing 10000 literals.

%This experiment shows that \system can achieve near-instant interactive response time with limited computing and storage resources. Even with minimal resources, the response time stays within the 0.6 second range, which---while not instant--- is still very usable. The takeaway message is that as long as indexing is affordable, as many literals as possible can be indexed, when indexing is no longer affordable, utilizing more computing resources can still preserve a good response time for \system. 

%As explained in Section~\ref{sec:pum}, searching for suggestions to complete the user's query involves searching a selected number of bins, and these bins are selected based on the length of the term written by the user. Our evaluation shows that the average filtering percentage is 46\%. This means that nearly half of the search space is excluded from the search task


\subsection{QSM Performance}

% \begin{table}[t]
%  \centering
%  \begin{tabular}{c c c c}
% \hline\hline
%  & Alt. Predicates & Alt. Literals & Relax Query \\ [0.5ex]
%  \hline
%  Percentage & 28\% & 17\% & 67\%\\
%  \hline
%  \end{tabular}
% \caption{The percentage of questions in which a QSM task was used in to find answers.}
% \label{tab:qsmPercentage}
% \end{table}

\begin{figure}[t]
\centering
\includegraphics[height=3.5cm,width=0.9\columnwidth]{figures/QuerySuggestionStages.pdf}
\caption{Average time required for different QSM tasks.}
\label{fig:suggestions}
\end{figure}

The logs of our user study indicate that participants used the suggestions
of the  QSM in over 90\% of the questions.
%The QSM suggests alternative predicates, alternaive literals, and relaxed query structure.
Users utilized
alternative predicates in 28\% of the questions,
alternative literals in 17\% of the questions,
and relaxed query structure in 67\% of the questions.
This demonstrates the crucial role the QSM plays in guiding the user towards correctly describing her questions.

Figure~\ref{fig:suggestions} shows the average execution time of each of the tasks in the QSM. That is, finding alternative predicates, finding alternative literals, relaxing the query, and answering the suggested queries.
As expected, answering the suggested queries takes the most time (around 7 seconds on average) since this step requires communicating to remote SPARQL endpoints.
% Answering one query takes 1.3 seconds on average, and the QSM needs to answer multiple suggested queries, leading to the 7 second total.
Adding up the time for the different tasks, we find that the QSM spends around 10 seconds on average before returning suggestions to the user. This is acceptable since the QSM does not interact with the user while she is typing. Instead, the user waits for suggestions from the QSM, and a 10 second wait is reasonable.

%Our experiments show that the participants used suggestions shown by the QSM in over 90\% of the questions. Table~\ref{tab:qsmPercentage} shows the percentage of questions where a task of the QSM was used to find answers for. The table shows that all tasks are important to find answers to most questions. It shows that the query relaxation is the task that is involved the most, whereas finding alternative literals task is the least involved, but it is still involved in approximately 17\% of the questions. This table demonstrates the crucial role the QSM plays in guiding the user to correctly describe her questions.

%Figure~\ref{fig:suggestions} shows the average execution time of each of the tasks in the QSM. That is, finding alternative predicates, finding alternative literals, relaxing the query, and answering alternative queries. The figure shows that answering alternative queries takes most of the time before returning suggestions to the user. We find that the average execution time for running a remote query is $1.3$ seconds, and answering alternative queries takes over 7 seconds per question on average. This is expected given that the generated alternative queries are executed remotely to provide the user with useful suggestions. Our experiments show that the average execution time spent by the QSM before returning suggestions is $10$ seconds.

